AutoConv: Automatically Generating Information-seeking Conversations with Large Language Models

Information-seeking conversation, which aims to help users gather information through conversation, has achieved great progress in recent years. However, the research is still stymied by the scarcity of training data. To alleviate this problem, we propose AutoConv for synthetic conversation generation, which takes advantage of the few-shot learning ability and generation capacity of large language models (LLM). Specifically, we formulate the conversation generation problem as a language modeling task, then finetune an LLM with a few human conversations to capture the characteristics of the information-seeking process and use it for generating synthetic conversations with high quality. Experimental results on two frequently-used datasets verify that AutoConv has substantial improvements over strong baselines and alleviates the dependence on human annotation. In addition, we also provide several analysis studies to promote future research.

==> tables/case_study.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3mm}        % 控制列间距
\begin{tabular}{m{1.5cm}m{13.0cm}}
\toprule
\multicolumn{1}{l}{\textbf{Title}} & 2006-2007: Ciara: The Evolution and acting debut                                   \\ \midrule
\multicolumn{1}{l}{\textbf{Document}} &
  On December 5, 2006, Ciara released her second studio album, Ciara: The Evolution. According to the singer, the title of the album is \textbackslash{}"about so much more than just my personal growth - it's about the evolution of music, the evolution of dance, the evolution of fashion.\textbackslash{}"The source of the album's creativity such as the sound and edge comes from Ciara in general.... Ciara: The Evolution became Ciara's first number one album on the U.S. Billboard 200 and second on the Top R\&B/Hip-Hop Albums ... \\ \midrule
\multicolumn{1}{l}{\multirow{14}{*}{\textbf{Dialogue}}} & Usr:\begin{tabular}{m{12.1cm}}What was the evolution?\end{tabular}                                         \\ \cmidrule(l){2-2} 
                           & Sys:\begin{tabular}{m{12.1cm}}On December 5, 2006, Ciara released her second studio album, Ciara: The Evolution.\end{tabular} \\ \cmidrule(l){2-2} 
                           & Usr:\begin{tabular}{m{12.1cm}}What was the name of the album?\end{tabular}                                                    \\ \cmidrule(l){2-2} 
 &
  Sys:\begin{tabular}{m{12.1cm}}The title of the album is \textbackslash{}"about so much more than just my personal growth - it's about the evolution of music, the evolution of dance, the evolution of fashion.\textbackslash{}"\end{tabular} \\ \cmidrule(l){2-2} 
                           & Usr:\begin{tabular}{m{12.1cm}}Did the album do well?\end{tabular}                                                           \\ \cmidrule(l){2-2} 
 &
  Sys:\begin{tabular}{m{12.1cm}}The album became Ciara's first number one album on the U.S. Billboard 200 and second on the Top R\&B/Hip-Hop Albums charts with sales of more than 338,000.\end{tabular} \\ \cmidrule(l){2-2} 
                           & Usr:\begin{tabular}{m{12.1cm}}What awards did she win if any?\end{tabular}                                                    \\ \cmidrule(l){2-2} 
 &
  Sys:\begin{tabular}{m{12.1cm}}
  The album went on to be certified platinum by the RIAA in the United States, within only five weeks of its release, and has sold 1.3 million copies according to Nielsen SoundScan.
\end{tabular} \\ \cmidrule(l){2-2} 
                           & Usr:\begin{tabular}{m{12.1cm}}What else did she accomplish during that time?\end{tabular}                                    \\ \cmidrule(l){2-2} 
                           & Sys:\begin{tabular}{m{12.1cm}}In support of the album, Ciara went on her first headlining tour in October 2006.\end{tabular}  \\ \cmidrule(l){2-2} 
                           & Usr:\begin{tabular}{m{12.1cm}}How long was the tour?\end{tabular}                                                             \\ \cmidrule(l){2-2} 
                           & Sys:\begin{tabular}{m{12.1cm}}The tour went to seventeen different clubs in cities throughout the United States.\end{tabular} \\ \cmidrule(l){2-2} 
                           & Usr:\begin{tabular}{m{12.1cm}}Did she have success with any songs?\end{tabular}                                               \\ \cmidrule(l){2-2} 
 &
  Sys:\begin{tabular}{m{12.1cm}}The lead single, \textbackslash{}"Get Up\textbackslash{}", which features Chamillionaire, reached number seven in the United States and gained a platinum accreditation.\end{tabular} \\ \bottomrule
\end{tabular}
\caption{An example of the synthetic conversation generated by AutoConv, the LLM is finetuned with 50 human dialogues from QuAC \cite{DBLP:conf/emnlp/ChoiHIYYCLZ18}.}
\label{tab:case_study}
\end{table*}
